Learning a Control Policy for Fall Prevention on an Assistive Walking Device

Fall prevention is one of the most important components in senior care. We present a technique to augment an assistive walking device with the ability to prevent falls. Given an existing walking device, our method develops a fall predictor and a recovery policy by utilizing the onboard sensors and actuators. The key component of our method is a robust human walking policy that models realistic human gait under a moderate level of perturbations. We use this human walking policy to provide training data for the fall predictor, as well as to teach the recovery policy how to best modify the person's gait when a fall is imminent. Our evaluation shows that the human walking policy generates walking sequences similar to those reported in biomechanics literature. Our experiments in simulation show that the augmented assistive device can indeed help recover balance from a variety of external perturbations. We also provide a quantitative method to evaluate the design choices for an assistive device.

==> Result.tex <==
\section{Results}
\label{sec:results}





==> exp.tex <==
\section{Experiments and Results}
\begin{figure}[!htpb]
%\centering
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{0.7}
\begin{tabular}{c c c c}
  \hline
  \includegraphics[width=0.1\textwidth,height=2cm]{images/phase0.png}&
  \includegraphics[width=0.1\textwidth,height=2cm]
  {images/phase1.png}&
  \includegraphics[width=0.1\textwidth,height=2cm]{images/phase3.png}&
  \includegraphics[width=0.1\textwidth,height=2cm]{images/phase4.png} \\ 
  \hline  
\end{tabular}
\caption{ This figure illustrates the 4 different timing of the left leg swing phase during which we test the performance of the exoskeleton. 
    }
\label{fig:phaseDefinition}
\end{figure}



\label{sec:Exp}

\begin{table}
\caption{Exoskeleton parameters}
\centering
\begin{tabular}{|l|l|}
\hline
 Torque Limits & 30 Nm  \\ \hline
 Sensors & IMU and Hip Joint Angle  \\ \hline
 Sensor delay & 40 - 50 ms \\ \hline
\end{tabular}
\label{tab:exo}
\end{table}

We validate the proposed framework using the open-source physics engine DART[DART].
Our humanoid model has $29$ degrees of freedom and its weight is $80$~Kg.
We also include the simulation model of the exoskeleton reported in [???], which connected to the humanoid with position constraints at hips \sehoon{something like this...}. 
We listed additional parameters of the exoskeleton model in \tabref{exo}.
For all experiments, the simulation time step is set to $0.002$s.
% The additional exoskeleton parameters are defined in table \ref{tab:exo}.
% physics engine to simulate a 29 DoF humanoid character as shown in figure \ref{fig:Dart}. The mass of the character is 80 Kg. We include exoskeleton design reported in \cite{}, to simulate the inertial effects of an exoskeleton on the human character. 
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/FootPlacements.png}
\caption{Comparison of the foot placement learned by the recovery policy and predicted by the model fitted using human motion capture data in (\cite{Wang2014}). The test is performed for 4 different pushes which induces different changes in the CoM velocities. In all the 4 cases, the step lengths are close with an maximum error of 2 cm. Only sagital plane pushes were considered in these experiments.}
\label{fig:manoj}
\end{figure}




We design experiments to systematically validate the learned human behaviors and effectiveness of the exoskeleton policy. In particular, our goal is to answer the following questions:
\begin{enumerate}
    \item Is the learned behavior of the human policy similar to data in the bio-mechanics literature?
    \item Does the exoskeleton policy improve the robustness of the gaits to external pushes?
    \item How does the effectiveness of the exoskeleton change with design choices?
\end{enumerate}

% We designed experiments to systematically evaluate all aspects of our approach : learnt behaviour of the human policy, effectiveness of the exoskeleton policy to help in recovery when the human policy fails and then we analyse the factors affecting the effectiveness of the policy. We identified that the first step to validate our approach is to compare the learned recovery behaviour of the human policy to data generated in bio-mechanics experiments with human subjects. Doing this will provide a strong basis to visually and statistically justify the close resemblance of the behaviour learned by the simulated character and the behaviour we observe in humans.
% More specifically these are the questions we hope to answer : 
% \begin{enumerate}
%     \item How does the learned behaviour of the policy compare to data collected from human studies in bio-mechanics literature?
%     \item How effective is the exoskeleton policy in helping with recovery when the human policy fails?
%     \item How does the effectiveness of the exoskeleton policy change with factors such as different sensor information and actuation capability.
% \end{enumerate}


\subsection{Comparison to observed human behaviour}
 


The performance of the exoskeleton must be evaluated on the realistic human behaviors because it involves two-way coupling between the human and exoskeleton.
In this section, our goal is to compare the learned human policy in \secref{human_policy}.



First, we validate the steady walking behavior of the human policy by comparing it to the data reported in \cite{Winter}.
\figref{Tauloops} illustrates the torque loops, the torque over joint angle, at the hip joint during a single gait cycle. 
We compute the torque loop of the learned policy directly using the simulation, while the ground truth data is collected by applying the inverse dynamics to the nominal human gait.
Although they are not identical, both trajectories formulate loops during a single gait cycle indicating energy being added and removed during the cycle.
In addition, we compare the joint angles during one cycle at the hip and knee joints (\figref{Jangles}).
From the figure, we verify that the joint trajectories of the simulated human are well matched to the data reported in \cite{Winter}.

In addition, we compare adjusted foot step locations due to external perturbations, which is comprehensively studied by Wang \etal \cite{Wang2014}.
Their findings strongly indicate that the COM dynamics is crucial in finding the next step placement which will help regain balance after a push.
They identified a model which predicts the changes in $x$ and $y$ location of the foot placement of a normal gait, $\delta_x$ and $\delta_y$, as a function of the COM velocity.
We compare this model against the foot step placements of the learned human policy.
\figref{fig:manoj} illustrates the foot placements of our model and the model of Wang \etal against four different magnitudes of pushes in the sagittal plane.
For all scenarios, the displacement error is below $?.??$~cm, which indicates that the learned human policy exhibits similar behaviors to a real human.

% Wang et al \cite{Wang2014} provided a comprehensive study on how foot placements are affected during external pushes on a steady state walking gait. Their findings strongly indicate that the CoM dynamics is crucial in finding the next step placement which will help regain balance after a push. They identified a model which predicts the $\delta_x$ and $\delta_y$, change in $x$ and $y$ location of the foot placement of a normal gait, as a function of the CoM velocity. We compare the foot placements learned by the recovery policy to that of the foot placements predicted by the model, and for sagital plane pushes to the CoM there is a close relationship between both of them. Figure \ref{fig:manoj} demonstrates this, we compare the foot placements for 4 different pushes which induce different changes in the CoM velocities. We believe that this is extremely useful result, because it confirms our hypothesis that the learned actions agrees well with human actions, and gives us confidence that our modelling of the human behaviour is reasonable.















\begin{comment}
\begin{figure}[th!]
\centering
\includegraphics[width=\linewidth]{images/TorqueLoops.png}

\caption{} 

\label{fig:loops}

\end{figure}

\begin{figure}[th!]
\centering
\includegraphics[width=\linewidth]{images/COmpare.png}

\caption{} 

\label{fig:JA}

\end{figure}
\end{comment}









\subsection{Effectiveness of exoskeleton policy}


To quantify the effectiveness of the exoskeleton policy in enabling recovery from an external push, we define a region of stability as shown in figure \ref{fig:exohelp}.This region, described by a polygon, defines the boundary of the maximum force applied at different angles in the x-y plane within which the policy can successfully recover. The region is computed by generating more rollouts of the policy after convergence. For every angle of push, we perform a line-search to identify the maximum force and this point becomes the vertex of the polygon. The region of stability gives us a good indication of the benefit of exoskeleton policy. Since, an external disturbance can be applied during any moment of the gait cycle, to standardize our experiments, we apply forces when the left leg is in the swing phase, as described in figure \ref{fig:phaseDefinition}. Due to this, we can notice that the area in the positive quadrant of the plots is larger. Figure \ref{fig:exohelp} illustrates the clear benefit of using an exoskeleton in aiding recovery motion. Figure \ref{fig:s} also shows one example of the recovery motion generated with the help of exoskeleton.

In addition to the region of stability, figures  describe the power usage of exoskeletons during the motion. The power plots help us understand the actions chosen by the exoskeleton policy that helps in successful recovery.  As figure \ref{fig:Power} illustrates, the additional torques applied by the exoskeleton at the hips help in recovery.




\subsection{Ablation Study}

As described in the previous section, although exoskeletons help in recovering balance, it is important to study the factors that affects the performance of the exoskeleton. For example, identifying appropriate sensor information and actuation capability required to achieve best recovery performance by the exoskeleton. In our ablation study, we learn 6 different exoskeleton policies, each policy has an input and actuation chosen from three different sensor inputs and actuation capability at the hip. We choose the area of the region of stability as a measure of the performance of each policy. Larger the area then more capable the exoskeleton is of enabling recovery. 


Figure \ref{fig:ActuationComp} compares the performance of two types of hip exoskeletons. $2D$ hip exoskeleton can actuate the hips only in the sagital plane, where as $3D$ hip exoskeletons can actuate the hip in both the sagital and frontal plane. $3D$ hip exoskeleton has a larger region of stability. This is reasonable because the additional degree of freedom in the frontal plane enables the exoskeleton to recover from a wider range of angles. 

Another important factor affecting the performance of exoskeleton is the sensory input to the policy. We compare three different types of input : 1) COM velocity and acceleration and hip joint angles, 2) Only CoM velocity and acceleration and 3) Only Hip joint angles. These are the most commonly used sensory information for a exoskeleton system, because they can be measured using Inertial measurement units (IMU's) and joint angle sensors. There has been some studies on using Electromyography (EMG) sensors as input to exoskeleton controllers, but due to the difficulty in simulating EMG sensors we leave it for future work. The goal of evaluating the exoskeleton performance with different inputs is to identify the kind of sensors needed to design effective exoskeletons. We learn 6 different exoskeleton policies with 3 different sensory inputs and 2 different actuation capabilities (3D and 2D). Figure , reveals that the exoskeleton with COM information plus hip proprioception performs best, this makes intuitive sense because both these pieces of information are needed to distinguish between states that have the same COM velocity/acceleration but are at a different phase of the gait cycle. 

Our experiments also lead to a important observation about the learned behaviour of the exoskeleton policy. During testing, we generate the region of stability plots when the forces are being applied at 4 different phases of the left leg swing phase, these 4 different timings are shown in figure \ref{fig:phaseDefinition}. Given the constraints such as torque limits, sensing capabilities and sensing delays the exoskeleton policy performs the best at phase 1 and the worst at phase 3. Phase 3 is the stage where the left leg is just about to strike the heel, at this point it is hard for the policy to find an action to adjust to the external disturbance because of the lack of time to react.  






